Jammer classification with Federated Learning

Jamming signals can jeopardize the operation of GNSS receivers until denying its operation. Given their ubiquity, jamming mitigation and localization techniques are of crucial importance, for which jammer classification is of help. Data-driven models have been proven useful in detecting these threats, while their training using crowdsourced data still poses challenges when it comes to private data sharing. This article investigates the use of federated learning to train jamming signal classifiers locally on each device, with model updates aggregated and averaged at the central server. This allows for privacy-preserving training procedures that do not require centralized data storage or access to client local data. The used framework FedAvg is assessed on a dataset consisting of spectrogram images of simulated interfered GNSS signal. Six different jammer types are effectively classified with comparable results to a fully centralized solution that requires vast amounts of data communication and involves privacy-preserving concerns.

==> images/dir01_accuracy.tex <==
% \documentclass[tikz]{standalone}

% \usepackage{pgfplots,siunitx,mathtools}

% \pgfplotsset{compat=newest}

% \begin{document}


\begin{tikzpicture}
  \begin{axis}[
    %   ymode=log,
      domain=1:33,
    %   ymax=0.9,
      enlargelimits=false,
      ylabel= Accuracy of Test/Global,
      xlabel= $q_0$,
      xtick={1,10,20,30,40,50,60,70,80,90,100},
      xticklabels={1,10,20,30,40,50,60,70,80,90,100}, %1.2,1.6,
      grid=both,
      width=9cm,
      height=5.5cm,
      decoration={name=none},
      legend style={at={(1,0)},anchor=south east}
    ]
%     \addplot [thick, smooth, green!70!black] coordinates {
%       (1, 0.5860000000000001)
% (2, 0.579)
% (3, 0.6466666666666667)
% (4, 0.6406666666666667)
% (5, 0.6846666666666665)
% (6, 0.7106666666666667)
% (7, 0.76)
% (8, 0.7843333333333333)
% (9, 0.7779999999999999)
%       }  node[pos=0.95, anchor=east];
    \addplot [thick, smooth, magenta!85!black] coordinates {
   (1, 60.765306122448976)
(2, 63.41836734693877)
(3, 62.55102040816327)
(4, 65.61224489795919)
(5, 65.35714285714286)
(6, 51.734693877551024)
(7, 81.93877551020408)
(8, 82.39795918367346)
(9, 81.88775510204081)
(10, 82.09183673469387)
(11, 84.59183673469387)
(12, 85.10204081632654)
(13, 85.86734693877551)
(14, 84.18367346938776)
(15, 84.08163265306122)
(16, 85.45918367346938)
(17, 85.61224489795919)
(18, 85.91836734693878)
(19, 85.3061224489796)
(20, 85.86734693877551)
(21, 85.66326530612245)
(22, 85.76530612244898)
(23, 87.09183673469387)
(24, 86.68367346938776)
(25, 86.42857142857143)
(26, 86.73469387755102)
(27, 86.3265306122449)
(28, 87.65306122448979)
(29, 86.78571428571429)
(30, 87.24489795918367)
(31, 87.65306122448979)
(32, 87.09183673469387)
(33, 87.60204081632654)
(34, 88.16326530612245)
(35, 87.60204081632654)
(36, 88.16326530612245)
(37, 88.57142857142857)
(38, 88.46938775510205)
(39, 88.9795918367347)
(40, 88.77551020408163)
(41, 88.9795918367347)
(42, 88.8265306122449)
(43, 89.18367346938776)
(44, 89.13265306122449)
(45, 88.46938775510205)
(46, 89.23469387755102)
(47, 88.6734693877551)
(48, 89.23469387755102)
(49, 89.64285714285714)
(50, 89.38775510204081)
(51, 89.43877551020408)
(52, 89.38775510204081)
(53, 89.74489795918367)
(54, 88.87755102040816)
(55, 89.84693877551021)
(56, 89.54081632653062)
(57, 89.89795918367346)
(58, 89.89795918367346)
(59, 89.74489795918367)
(60, 89.74489795918367)
(61, 89.6938775510204)
(62, 90.05102040816327)
(63, 90.10204081632654)
(64, 89.84693877551021)
(65, 90.25510204081633)
(66, 89.84693877551021)
(67, 90.51020408163264)
(68, 90.25510204081633)
(69, 90.05102040816327)
(70, 90.20408163265306)
(71, 90.6122448979592)
(72, 90.6122448979592)
(73, 90.6122448979592)
(74, 90.91836734693878)
(75, 90.71428571428572)
(76, 90.6122448979592)
(77, 90.51020408163264)
(78, 90.76530612244898)
(79, 91.07142857142856)
(80, 91.0204081632653)
(81, 90.86734693877553)
(82, 90.66326530612244)
(83, 90.86734693877553)
(84, 91.1734693877551)
(85, 91.07142857142856)
(86, 91.27551020408164)
(87, 91.07142857142856)
(88, 91.1734693877551)
(89, 91.22448979591836)
(90, 91.27551020408164)
(91, 91.63265306122447)
(92, 91.3265306122449)
(93, 91.12244897959184)
(94, 91.53061224489797)
(95, 91.53061224489797)
(96, 91.53061224489797)
(97, 91.1734693877551)
(98, 91.58163265306122)
(99, 91.37755102040816)
(100, 91.68367346938776)
    }node[pos=0.95, anchor=east] {};
    \addplot [thick, smooth, cyan!70!black] coordinates {
        (1, 17.31358529111338)
(2, 32.63534218590399)
(3, 30.949948927477017)
(4, 30.541368743615934)
(5, 31.256384065372828)
(6, 31.05209397344229)
(7, 31.869254341164453)
(8, 32.58426966292135)
(9, 35.95505617977528)
(10, 34.32073544433095)
(11, 46.37385086823289)
(12, 42.64555669050051)
(13, 44.73953013278856)
(14, 48.67211440245149)
(15, 52.34933605720123)
(16, 47.95709908069458)
(17, 61.28702757916241)
(18, 60.52093973442288)
(19, 58.631256384065374)
(20, 64.14708886618999)
(21, 68.07967313585291)
(22, 69.76506639427988)
(23, 66.1899897854954)
(24, 68.89683350357508)
(25, 74.41266598569969)
(26, 72.9826353421859)
(27, 66.54749744637385)
(28, 74.51481103166496)
(29, 72.01225740551584)
(30, 75.4341164453524)
(31, 77.52808988764045)
(32, 77.3237997957099)
(33, 78.6006128702758)
(34, 75.74055158324822)
(35, 76.60878447395301)
(36, 78.08988764044943)
(37, 78.39632277834525)
(38, 79.41777323799796)
(39, 78.34525025536261)
(40, 78.49846782431052)
(41, 79.41777323799796)
(42, 80.08171603677222)
(43, 79.82635342185904)
(44, 81.00102145045965)
(45, 81.00102145045965)
(46, 81.05209397344228)
(47, 80.13278855975486)
(48, 80.69458631256384)
(49, 81.66496424923392)
(50, 81.92032686414709)
(51, 81.46067415730337)
(52, 79.26455566905005)
(53, 73.34014300306436)
(54, 80.69458631256384)
(55, 81.76710929519918)
(56, 81.3585291113381)
(57, 81.76710929519918)
(58, 80.84780388151175)
(59, 82.63534218590398)
(60, 83.70786516853933)
(61, 82.2267620020429)
(62, 81.30745658835546)
(63, 80.28600612870275)
(64, 82.68641470888662)
(65, 82.073544433095)
(66, 82.83963227783453)
(67, 82.89070480081716)
(68, 83.2482124616956)
(69, 81.66496424923392)
(70, 83.45250255362615)
(71, 83.45250255362615)
(72, 83.9632277834525)
(73, 83.65679264555669)
(74, 83.0949948927477)
(75, 82.73748723186925)
(76, 83.40143003064351)
(77, 73.49336057201226)
(78, 81.97139938712972)
(79, 65.21961184882534)
(80, 82.48212461695607)
(81, 82.73748723186925)
(82, 83.91215526046987)
(83, 83.91215526046987)
(84, 83.70786516853933)
(85, 83.75893769152196)
(86, 84.32073544433095)
(87, 83.65679264555669)
(88, 84.72931562819203)
(89, 84.37180796731359)
(90, 82.43105209397345)
(91, 85.34218590398366)
(92, 84.5250255362615)
(93, 84.93360572012257)
(94, 84.42288049029622)
(95, 84.98467824310521)
(96, 84.93360572012257)
(97, 84.98467824310521)
(98, 84.8314606741573)
(99, 68.99897854954035)
(100, 84.42288049029622)
      }  node[pos=0.95, anchor=east] {};
%       \addplot [thick, smooth, dashed, green!70!black] coordinates {
%         (1, 0.6323333333333333)
% (2, 0.6733333333333333)
% (3, 0.7169999999999999)
% (4, 0.7443333333333332)
% (5, 0.82725)
% (6, 0.86525)
% (7, 0.8767499999999999)
% (8, 0.8944999999999999)
% (9, 0.8827500000000001)
%       }  node[pos=0.95, anchor=east];
      \addplot [thick, smooth, dashed, magenta!70!black] coordinates {
        (1, 30.40816326530612)
(2, 47.704081632653065)
(3, 52.704081632653065)
(4, 62.6530612244898)
(5, 38.41836734693877)
(6, 38.41836734693877)
(7, 55.56122448979592)
(8, 56.224489795918366)
(9, 67.14285714285714)
(10, 60.96938775510204)
(11, 61.07142857142857)
(12, 72.39795918367346)
(13, 65.81632653061224)
(14, 63.826530612244895)
(15, 73.57142857142857)
(16, 76.3265306122449)
(17, 76.58163265306122)
(18, 74.18367346938776)
(19, 79.13265306122449)
(20, 78.06122448979592)
(21, 78.41836734693878)
(22, 76.73469387755102)
(23, 81.58163265306122)
(24, 81.98979591836735)
(25, 81.4795918367347)
(26, 81.37755102040816)
(27, 82.70408163265306)
(28, 84.74489795918367)
(29, 83.16326530612245)
(30, 82.75510204081633)
(31, 83.46938775510205)
(32, 83.16326530612245)
(33, 84.6938775510204)
(34, 85.61224489795919)
(35, 83.57142857142857)
(36, 83.5204081632653)
(37, 86.42857142857143)
(38, 85.81632653061224)
(39, 86.27551020408163)
(40, 86.63265306122449)
(41, 86.63265306122449)
(42, 85.96938775510205)
(43, 86.42857142857143)
(44, 86.73469387755102)
(45, 85.86734693877551)
(46, 86.27551020408163)
(47, 85.96938775510205)
(48, 86.22448979591837)
(49, 86.93877551020408)
(50, 86.68367346938776)
(51, 84.59183673469387)
(52, 86.12244897959184)
(53, 87.04081632653062)
(54, 84.6938775510204)
(55, 86.53061224489795)
(56, 86.58163265306122)
(57, 86.37755102040816)
(58, 86.78571428571429)
(59, 86.58163265306122)
(60, 85.56122448979592)
(61, 86.27551020408163)
(62, 87.04081632653062)
(63, 87.90816326530613)
(64, 86.37755102040816)
(65, 86.68367346938776)
(66, 86.37755102040816)
(67, 87.39795918367346)
(68, 86.98979591836735)
(69, 86.1734693877551)
(70, 86.78571428571429)
(71, 86.88775510204081)
(72, 88.26530612244898)
(73, 87.5)
(74, 88.01020408163265)
(75, 87.90816326530613)
(76, 87.95918367346938)
(77, 87.24489795918367)
(78, 87.34693877551021)
(79, 87.29591836734694)
(80, 87.29591836734694)
(81, 86.88775510204081)
(82, 86.53061224489795)
(83, 87.04081632653062)
(84, 87.65306122448979)
(85, 87.95918367346938)
(86, 88.16326530612245)
(87, 87.5)
(88, 88.26530612244898)
(89, 88.11224489795919)
(90, 87.24489795918367)
(91, 88.31632653061224)
(92, 87.90816326530613)
(93, 88.16326530612245)
(94, 87.95918367346938)
(95, 88.26530612244898)
(96, 88.57142857142857)
(97, 88.9795918367347)
(98, 88.57142857142857)
(99, 88.9795918367347)
(100, 88.5204081632653)
      }  node[pos=0.95, anchor=east] {};
      
    \legend{Global, Fedavg, Fedprox}
   \end{axis}
\end{tikzpicture} 

% \end{document}

==> images/iid_accuracy.tex <==
% \documentclass[tikz]{standalone}

% \usepackage{pgfplots,siunitx,mathtools}

% \pgfplotsset{compat=newest}

% \begin{document}


\begin{tikzpicture}
  \begin{axis}[
    %   ymode=log,
      domain=1:33,
    %   ymax=0.9,
      enlargelimits=false,
      ylabel= Accuracy of Test/Global,
      xlabel= $q_0$,
      xtick={1,10,20,30,40,50,60,70,80,90,100},
      xticklabels={1,10,20,30,40,50,60,70,80,90,100}, %1.2,1.6,
      grid=both,
      width=9cm,
      height=5.5cm,
      decoration={name=none},
      legend style={at={(1,0)},anchor=south east}
    ]
%     \addplot [thick, smooth, green!70!black] coordinates {
%       (1, 0.5860000000000001)
% (2, 0.579)
% (3, 0.6466666666666667)
% (4, 0.6406666666666667)
% (5, 0.6846666666666665)
% (6, 0.7106666666666667)
% (7, 0.76)
% (8, 0.7843333333333333)
% (9, 0.7779999999999999)
%       }  node[pos=0.95, anchor=east];
    \addplot [thick, smooth, magenta!85!black] coordinates {
   (1, 60.765306122448976)
(2, 63.41836734693877)
(3, 62.55102040816327)
(4, 65.61224489795919)
(5, 65.35714285714286)
(6, 51.734693877551024)
(7, 81.93877551020408)
(8, 82.39795918367346)
(9, 81.88775510204081)
(10, 82.09183673469387)
(11, 84.59183673469387)
(12, 85.10204081632654)
(13, 85.86734693877551)
(14, 84.18367346938776)
(15, 84.08163265306122)
(16, 85.45918367346938)
(17, 85.61224489795919)
(18, 85.91836734693878)
(19, 85.3061224489796)
(20, 85.86734693877551)
(21, 85.66326530612245)
(22, 85.76530612244898)
(23, 87.09183673469387)
(24, 86.68367346938776)
(25, 86.42857142857143)
(26, 86.73469387755102)
(27, 86.3265306122449)
(28, 87.65306122448979)
(29, 86.78571428571429)
(30, 87.24489795918367)
(31, 87.65306122448979)
(32, 87.09183673469387)
(33, 87.60204081632654)
(34, 88.16326530612245)
(35, 87.60204081632654)
(36, 88.16326530612245)
(37, 88.57142857142857)
(38, 88.46938775510205)
(39, 88.9795918367347)
(40, 88.77551020408163)
(41, 88.9795918367347)
(42, 88.8265306122449)
(43, 89.18367346938776)
(44, 89.13265306122449)
(45, 88.46938775510205)
(46, 89.23469387755102)
(47, 88.6734693877551)
(48, 89.23469387755102)
(49, 89.64285714285714)
(50, 89.38775510204081)
(51, 89.43877551020408)
(52, 89.38775510204081)
(53, 89.74489795918367)
(54, 88.87755102040816)
(55, 89.84693877551021)
(56, 89.54081632653062)
(57, 89.89795918367346)
(58, 89.89795918367346)
(59, 89.74489795918367)
(60, 89.74489795918367)
(61, 89.6938775510204)
(62, 90.05102040816327)
(63, 90.10204081632654)
(64, 89.84693877551021)
(65, 90.25510204081633)
(66, 89.84693877551021)
(67, 90.51020408163264)
(68, 90.25510204081633)
(69, 90.05102040816327)
(70, 90.20408163265306)
(71, 90.6122448979592)
(72, 90.6122448979592)
(73, 90.6122448979592)
(74, 90.91836734693878)
(75, 90.71428571428572)
(76, 90.6122448979592)
(77, 90.51020408163264)
(78, 90.76530612244898)
(79, 91.07142857142856)
(80, 91.0204081632653)
(81, 90.86734693877553)
(82, 90.66326530612244)
(83, 90.86734693877553)
(84, 91.1734693877551)
(85, 91.07142857142856)
(86, 91.27551020408164)
(87, 91.07142857142856)
(88, 91.1734693877551)
(89, 91.22448979591836)
(90, 91.27551020408164)
(91, 91.63265306122447)
(92, 91.3265306122449)
(93, 91.12244897959184)
(94, 91.53061224489797)
(95, 91.53061224489797)
(96, 91.53061224489797)
(97, 91.1734693877551)
(98, 91.58163265306122)
(99, 91.37755102040816)
(100, 91.68367346938776)
    }node[pos=0.95, anchor=east] {};
    \addplot [thick, smooth, cyan!70!black] coordinates {
        (1, 62.55102040816327)
(2, 64.79591836734694)
(3, 56.58163265306123)
(4, 66.73469387755102)
(5, 70.66326530612245)
(6, 55.40816326530612)
(7, 80.71428571428571)
(8, 81.63265306122449)
(9, 82.24489795918367)
(10, 81.88775510204081)
(11, 84.43877551020408)
(12, 84.84693877551021)
(13, 86.0204081632653)
(14, 83.87755102040816)
(15, 84.59183673469387)
(16, 85.71428571428571)
(17, 85.71428571428571)
(18, 86.0204081632653)
(19, 85.35714285714286)
(20, 86.0204081632653)
(21, 85.25510204081633)
(22, 85.86734693877551)
(23, 87.04081632653062)
(24, 86.93877551020408)
(25, 86.37755102040816)
(26, 86.83673469387755)
(27, 86.42857142857143)
(28, 87.60204081632654)
(29, 86.78571428571429)
(30, 87.1938775510204)
(31, 87.65306122448979)
(32, 86.88775510204081)
(33, 87.65306122448979)
(34, 88.01020408163265)
(35, 87.5)
(36, 88.06122448979592)
(37, 88.57142857142857)
(38, 88.26530612244898)
(39, 88.92857142857143)
(40, 88.57142857142857)
(41, 89.18367346938776)
(42, 88.72448979591837)
(43, 88.92857142857143)
(44, 89.28571428571429)
(45, 88.36734693877551)
(46, 89.23469387755102)
(47, 88.62244897959184)
(48, 89.13265306122449)
(49, 89.74489795918367)
(50, 89.38775510204081)
(51, 89.33673469387755)
(52, 89.54081632653062)
(53, 89.84693877551021)
(54, 88.6734693877551)
(55, 89.84693877551021)
(56, 89.48979591836735)
(57, 90.0)
(58, 90.0)
(59, 89.74489795918367)
(60, 89.6938775510204)
(61, 89.84693877551021)
(62, 90.1530612244898)
(63, 90.10204081632654)
(64, 89.64285714285714)
(65, 90.20408163265306)
(66, 89.79591836734694)
(67, 90.6122448979592)
(68, 90.35714285714286)
(69, 90.25510204081633)
(70, 90.3061224489796)
(71, 90.76530612244898)
(72, 90.51020408163264)
(73, 90.71428571428572)
(74, 91.07142857142856)
(75, 90.81632653061224)
(76, 90.96938775510203)
(77, 90.66326530612244)
(78, 90.6122448979592)
(79, 90.96938775510203)
(80, 90.86734693877553)
(81, 91.0204081632653)
(82, 90.81632653061224)
(83, 90.96938775510203)
(84, 91.1734693877551)
(85, 91.12244897959184)
(86, 91.3265306122449)
(87, 91.22448979591836)
(88, 91.27551020408164)
(89, 91.1734693877551)
(90, 91.1734693877551)
(91, 91.58163265306122)
(92, 91.3265306122449)
(93, 91.3265306122449)
(94, 91.4795918367347)
(95, 91.63265306122447)
(96, 91.58163265306122)
(97, 91.07142857142856)
(98, 91.53061224489797)
(99, 91.3265306122449)
(100, 91.53061224489797)
      }  node[pos=0.95, anchor=east] {};
%       \addplot [thick, smooth, dashed, green!70!black] coordinates {
%         (1, 0.6323333333333333)
% (2, 0.6733333333333333)
% (3, 0.7169999999999999)
% (4, 0.7443333333333332)
% (5, 0.82725)
% (6, 0.86525)
% (7, 0.8767499999999999)
% (8, 0.8944999999999999)
% (9, 0.8827500000000001)
%       }  node[pos=0.95, anchor=east];
      \addplot [thick, smooth, dashed, magenta!70!black] coordinates {
        (1, 30.40816326530612)
(2, 47.704081632653065)
(3, 52.704081632653065)
(4, 62.6530612244898)
(5, 38.41836734693877)
(6, 38.41836734693877)
(7, 55.56122448979592)
(8, 56.224489795918366)
(9, 67.14285714285714)
(10, 60.96938775510204)
(11, 61.07142857142857)
(12, 72.39795918367346)
(13, 65.81632653061224)
(14, 63.826530612244895)
(15, 73.57142857142857)
(16, 76.3265306122449)
(17, 76.58163265306122)
(18, 74.18367346938776)
(19, 79.13265306122449)
(20, 78.06122448979592)
(21, 78.41836734693878)
(22, 76.73469387755102)
(23, 81.58163265306122)
(24, 81.98979591836735)
(25, 81.4795918367347)
(26, 81.37755102040816)
(27, 82.70408163265306)
(28, 84.74489795918367)
(29, 83.16326530612245)
(30, 82.75510204081633)
(31, 83.46938775510205)
(32, 83.16326530612245)
(33, 84.6938775510204)
(34, 85.61224489795919)
(35, 83.57142857142857)
(36, 83.5204081632653)
(37, 86.42857142857143)
(38, 85.81632653061224)
(39, 86.27551020408163)
(40, 86.63265306122449)
(41, 86.63265306122449)
(42, 85.96938775510205)
(43, 86.42857142857143)
(44, 86.73469387755102)
(45, 85.86734693877551)
(46, 86.27551020408163)
(47, 85.96938775510205)
(48, 86.22448979591837)
(49, 86.93877551020408)
(50, 86.68367346938776)
(51, 84.59183673469387)
(52, 86.12244897959184)
(53, 87.04081632653062)
(54, 84.6938775510204)
(55, 86.53061224489795)
(56, 86.58163265306122)
(57, 86.37755102040816)
(58, 86.78571428571429)
(59, 86.58163265306122)
(60, 85.56122448979592)
(61, 86.27551020408163)
(62, 87.04081632653062)
(63, 87.90816326530613)
(64, 86.37755102040816)
(65, 86.68367346938776)
(66, 86.37755102040816)
(67, 87.39795918367346)
(68, 86.98979591836735)
(69, 86.1734693877551)
(70, 86.78571428571429)
(71, 86.88775510204081)
(72, 88.26530612244898)
(73, 87.5)
(74, 88.01020408163265)
(75, 87.90816326530613)
(76, 87.95918367346938)
(77, 87.24489795918367)
(78, 87.34693877551021)
(79, 87.29591836734694)
(80, 87.29591836734694)
(81, 86.88775510204081)
(82, 86.53061224489795)
(83, 87.04081632653062)
(84, 87.65306122448979)
(85, 87.95918367346938)
(86, 88.16326530612245)
(87, 87.5)
(88, 88.26530612244898)
(89, 88.11224489795919)
(90, 87.24489795918367)
(91, 88.31632653061224)
(92, 87.90816326530613)
(93, 88.16326530612245)
(94, 87.95918367346938)
(95, 88.26530612244898)
(96, 88.57142857142857)
(97, 88.9795918367347)
(98, 88.57142857142857)
(99, 88.9795918367347)
(100, 88.5204081632653)
      }  node[pos=0.95, anchor=east] {};
      
    \legend{Global, Fedavg, Fedprox}
   \end{axis}
\end{tikzpicture} 

% \end{document}
